On the Importance of Firth Bias Reduction in Few-Shot Classification

Learning accurate classifiers for novel categories from very few examples, known as few-shot image classification, is a challenging task in statistical machine learning and computer vision. The performance in few-shot classification suffers from the bias in the estimation of classifier parameters; however, an effective underlying bias reduction technique that could alleviate this issue in training few-shot classifiers has been overlooked. In this work, we demonstrate the effectiveness of Firth bias reduction in few-shot classification. Theoretically, Firth bias reduction removes the $O(N^{-1})$ first order term from the small-sample bias of the Maximum Likelihood Estimator. Here we show that the general Firth bias reduction technique simplifies to encouraging uniform class assignment probabilities for multinomial logistic classification, and almost has the same effect in cosine classifiers. We derive an easy-to-implement optimization objective for Firth penalized multinomial logistic and cosine classifiers, which is equivalent to penalizing the cross-entropy loss with a KL-divergence between the uniform label distribution and the predictions. Then, we empirically evaluate that it is consistently effective across the board for few-shot image classification, regardless of (1) the feature representations from different backbones, (2) the number of samples per class, and (3) the number of classes. Finally, we show the robustness of Firth bias reduction, in the case of imbalanced data distribution. Our implementation is available at https://github.com/ehsansaleh/firth_bias_reduction

==> Discussion.tex <==
As empirically shown in the experiments, while it does not hurt the performance, Firth regularization does not bring as significant gains in 1-shot as in higher-shot scenarios.  This observation is in line with the fact that $1$-shot classification is intrinsically hard, especially when the number of classes increases. To address this challenge, we plan to investigate other under-explored regularization techniques for bias reduction in the low-data regime. In addition, it is very likely that in this extremely challenging 1-shot regime, feature learning and classifier learning should be jointly tackled towards the performance improvements. Future work will investigate these.

%In fact, training $1$-shot classifiers is so hard that the feature representation may be the only viable means towards its improvement. As Firth regularization seems to not be effective in the $1$-shot case, it motivates investigating other under-explored regularization techniques to address the bias issue in the few-shot setting for the future work.%seems to not be effective in the $1$-shot case,

%The experiments in Section~\ref{sec:cosineexp} indicate that in the $1$-shot task, the improvement by Firth regularization is monotonically decreasing with the number of classes in all the datasets except tiered-ImageNet, but it does not hurt the performance. The improvement almost falls within (0.1\%-0.5\%), (0-0.1\%), and (0-0.2\%), for mini-ImageNet, CIFAR-FS, and tiered-ImageNet, respectively. 

==> paper_tables/main/s2m2rf/tritbl_cifar_val2test_ci.tex <==
% \begin{table}[h]
%   \centering
%   \begin{tabular}{ccccccc}
%     \toprule
%             & \multicolumn{3}{c}{5-way} & \multicolumn{3}{c}{10-way} \\\midrule
%             & Before &        After &   Improvement & Before &        After &   Improvement \\\midrule
%     1-shot &  74.96 &  75.03 $\pm$ 0.19 &  0.07 $\pm$ 0.01 &  61.46 &  61.49 $\pm$ 0.13 &  0.03 $\pm$ 0.00 \\\midrule
%     5-shot &  87.43  &  87.48 $\pm$ 0.13 &  0.06 $\pm$ 0.00 &  77.73  &  77.83 $\pm$ 0.10 &  0.10 $\pm$ 0.00 \\\midrule
%     10-shot &  89.83 &  89.88 $\pm$ 0.11 &  0.05 $\pm$ 0.00 &  81.52 &  81.64 $\pm$ 0.09 &  0.11 $\pm$ 0.00 \\
%     \bottomrule
%     \end{tabular}\\ \vspace{0.45em}
%   \begin{tabular}{ccccccc}
%     \toprule
%             & \multicolumn{3}{c}{15-way} & \multicolumn{3}{c}{20-way} \\\midrule
%             & Before &        After &   Improvement & Before &        After &   Improvement \\\midrule
%     1-shot & 53.45 &  53.47 $\pm$ 0.10 &  0.02 $\pm$ 0.00 &  47.78 &  47.79 $\pm$ 0.07 &  0.01 $\pm$ 0.00 \\\midrule
%     5-shot & 70.70 &  70.99 $\pm$ 0.07 &  0.28 $\pm$ 0.00 &  65.26 &  65.60 $\pm$ 0.03 &  0.34 $\pm$ 0.00 \\\midrule
%     10-shot & 75.37 &  75.71 $\pm$ 0.06 &  0.34 $\pm$ 0.00 &  70.57 &  70.99 $\pm$ 0.02 &  0.42 $\pm$ 0.00 \\
%     \bottomrule
%     \end{tabular}
    
%   \caption{\textbf{The Firth bias reduction improvements on the CIFAR-FS dataset shown in Figure~\ref{fig:s2m2rf} of the main paper.} ``Before'' stands for the novel set accuracy without having any Firth bias reduction, and ``After'' stands for the novel set accuracy after applying Firth bias reduction. Note that the confidence intervals are much smaller for the improvement column thanks to the random-effect matching procedure we used in this study. The ``Before'' confidence intervals were similar to the ``After'' confidence intervals, and thus not repeated due to space constraints.}
%   \label{tab:s2m2cifarpart1}%
% \end{table}%

\begin{table}[h]
  \centering
  \begin{tabular}{ccccccc}
    \toprule
    & Before &        After &   Improvement & Before &        After &   Improvement \\\midrule
    & \multicolumn{3}{c}{5-way} & \multicolumn{3}{c}{10-way} \\\midrule
    1-shot &  74.96 &  75.03 $\pm$ 0.19 &  0.07 $\pm$ 0.01 &  61.46 &  61.49 $\pm$ 0.13 &  0.03 $\pm$ 0.00 \\\midrule
    5-shot &  87.43  &  87.48 $\pm$ 0.13 &  0.06 $\pm$ 0.00 &  77.73  &  77.83 $\pm$ 0.10 &  0.10 $\pm$ 0.00 \\\midrule
    10-shot &  89.83 &  89.88 $\pm$ 0.11 &  0.05 $\pm$ 0.00 &  81.52 &  81.64 $\pm$ 0.09 &  0.11 $\pm$ 0.00 \\\midrule
    & \multicolumn{3}{c}{15-way} & \multicolumn{3}{c}{20-way} \\\midrule
    1-shot & 53.45 &  53.47 $\pm$ 0.10 &  0.02 $\pm$ 0.00 &  47.78 &  47.79 $\pm$ 0.07 &  0.01 $\pm$ 0.00 \\\midrule
    5-shot & 70.70 &  70.99 $\pm$ 0.07 &  0.28 $\pm$ 0.00 &  65.26 &  65.60 $\pm$ 0.03 &  0.34 $\pm$ 0.00 \\\midrule
    10-shot & 75.37 &  75.71 $\pm$ 0.06 &  0.34 $\pm$ 0.00 &  70.57 &  70.99 $\pm$ 0.02 &  0.42 $\pm$ 0.00 \\
    \bottomrule
    \end{tabular}\\ \vspace{0.45em}
  \caption{\textbf{The Firth bias reduction improvements on the CIFAR-FS dataset shown in Figure~\ref{fig:s2m2rf} in the main paper.} ``Before'' stands for the novel set accuracy without having any Firth bias reduction, and ``After'' stands for the novel set accuracy after applying Firth bias reduction. Note that the confidence intervals are much smaller for the improvement column, thanks to the random-effect matching procedure we used in this study. The ``Before'' confidence intervals were similar to the ``After'' confidence intervals, and thus not repeated due to space constraints.}
  \label{tab:s2m2cifarpart1}%
\end{table}%


==> paper_tables/main/s2m2rf/tritbl_miniImagenet_val2test_ci.tex <==
\begin{figure}[t]
	\centering
	\includegraphics[width=0.96\linewidth]{paper_plots/appendix/embeddings/dacc_vs_nways_dn121_tiered.pdf}\\
	\includegraphics[width=0.96\linewidth]{paper_plots/appendix/embeddings/dacc_vs_nways_mn84_tiered.pdf}
	\caption{{Firth bias reduction improves the accuracy of the logistic classifier on tieredImageNet for both \textbf{DenseNet (top)} and \textbf{MobileNet (bottom)} as backbone architectures. The improvement is consistent over the number of classes in few-shot classification.} The error bars are almost non-existent (i.e., less than $0.02\%$), since over 10,000 trials with {matching randomization factors} were used for obtaining each single point. {Firth bias reduction} improvements are always positive, and it never hurts to use it.}
	\label{fig:simpleshot}
\end{figure}

% \begin{table}[h]
%   \centering
  
%     \begin{tabular}{ccccccc}
%     \toprule
%             & \multicolumn{3}{c}{5-way} & \multicolumn{3}{c}{10-way} \\\midrule
%             & Before &        After &   Improvement & Before &        After &   Improvement \\\midrule
%     1-shot &  65.17 &  {65.59}  $\pm$ 0.18 &  0.41 $\pm$ 0.02 &  50.38 &  {50.64} $\pm$ 0.11 &  0.26 $\pm$ 0.01\\\midrule
%     5-shot &  82.60 &  {83.04} $\pm$ 0.12 &  0.44 $\pm$ 0.01 &  71.15 &  {71.91} $\pm$ 0.10 &  0.76 $\pm$ 0.02\\\midrule
%     10-shot &  86.82 &  {87.04} $\pm$ 0.09  &  0.22 $\pm$ 0.01 &  77.34 &  {77.87}  $\pm$ 0.08 &  0.52 $\pm$ 0.01 \\
%     \bottomrule
%     \end{tabular}\\\vspace{0.45em}
    
    
%     \begin{tabular}{ccccccc}
%     \toprule
%             & \multicolumn{3}{c}{15-way} & \multicolumn{3}{c}{20-way} \\\midrule
%             & Before &        After &   Improvement & Before &        After &   Improvement \\\midrule
%     1-shot & 42.65 &  {42.85} $\pm$ 0.08 &  0.20 $\pm$ 0.01 &  37.56 &  {37.76} $\pm$ 0.07 &  0.20 $\pm$ 0.00 \\\midrule
%     5-shot & 63.73 &  {64.76} $\pm$ 0.07  &  1.03 $\pm$ 0.01 &  58.35 &  {59.52} $\pm$ 0.04 &  1.17 $\pm$ 0.01 \\\midrule
%     10-shot &  70.87 &  {71.71} $\pm$ 0.05  &  0.84 $\pm$ 0.01 &  66.06 &  {67.12} $\pm$ 0.03 &  1.06 $\pm$ 0.01 \\
%     \bottomrule
%     \end{tabular}

    
%   \caption{\textbf{The Firth bias reduction improvements on the mini-ImageNet dataset shown in Figure~\ref{fig:s2m2rf} of the main paper.} ``Before'' stands for the novel set accuracy without having any Firth bias reduction, and ``After'' stands for the novel set accuracy after applying Firth bias reduction. Note that the confidence intervals are much smaller for the improvement column thanks to the random-effect matching procedure we used in this study. The ``Before'' confidence intervals were similar to the ``After'' confidence intervals, and thus not repeated due to space constraints.}
%   \label{tab:s2m2minipart1}%
% \end{table}%

\begin{table}[h]
  \centering
  
    \begin{tabular}{ccccccc}
    \toprule
    & Before &        After &   Improvement & Before &        After &   Improvement \\\midrule
    & \multicolumn{3}{c}{5-way} & \multicolumn{3}{c}{10-way} \\\midrule
    1-shot &  65.17 &  {65.59}  $\pm$ 0.18 &  0.41 $\pm$ 0.02 &  50.38 &  {50.64} $\pm$ 0.11 &  0.26 $\pm$ 0.01\\\midrule
    5-shot &  82.60 &  {83.04} $\pm$ 0.12 &  0.44 $\pm$ 0.01 &  71.15 &  {71.91} $\pm$ 0.10 &  0.76 $\pm$ 0.02\\\midrule
    10-shot &  86.82 &  {87.04} $\pm$ 0.09  &  0.22 $\pm$ 0.01 &  77.34 &  {77.87}  $\pm$ 0.08 &  0.52 $\pm$ 0.01 \\\midrule
    & \multicolumn{3}{c}{15-way} & \multicolumn{3}{c}{20-way} \\\midrule
    1-shot & 42.65 &  {42.85} $\pm$ 0.08 &  0.20 $\pm$ 0.01 &  37.56 &  {37.76} $\pm$ 0.07 &  0.20 $\pm$ 0.00 \\\midrule
    5-shot & 63.73 &  {64.76} $\pm$ 0.07  &  1.03 $\pm$ 0.01 &  58.35 &  {59.52} $\pm$ 0.04 &  1.17 $\pm$ 0.01 \\\midrule
    10-shot &  70.87 &  {71.71} $\pm$ 0.05  &  0.84 $\pm$ 0.01 &  66.06 &  {67.12} $\pm$ 0.03 &  1.06 $\pm$ 0.01 \\
    \bottomrule
    \end{tabular}\\\vspace{0.45em}
  \caption{\textbf{The Firth bias reduction improvements on the mini-ImageNet dataset shown in Figure~\ref{fig:s2m2rf} of the main paper.} ``Before'' stands for the novel set accuracy without having any Firth bias reduction, and ``After'' stands for the novel set accuracy after applying Firth bias reduction. Note that the confidence intervals are much smaller for the improvement column thanks to the random-effect matching procedure we used in this study. The ``Before'' confidence intervals were similar to the ``After'' confidence intervals, and thus not repeated due to space constraints.}
  \label{tab:s2m2minipart1}%
\end{table}%

==> paper_tables/main/s2m2rf/tritbl_tieredImagenet2_val2test_ci.tex <==
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c}
\toprule
        & \multicolumn{3}{c|}{50-way} & \multicolumn{3}{c|}{100-way} & \multicolumn{3}{c|}{150-way} \\\midrule
        & Before &        After &   Improvement &  Before &        After &   Improvement &  Before &        After &   Improvement \\\midrule
\midrule
1-shot &  33.91 &  \textbf{34.13} &  0.22 $\pm$ 0.01 &   24.80 &  \textbf{25.00} &  0.20 $\pm$ 0.00 &   20.37 &  \textbf{20.56} &  0.19 $\pm$ 0.00 \\\midrule
5-shot &  52.60 &  \textbf{54.71} &  2.10 $\pm$ 0.01 &   41.03 &  \textbf{43.59} &  2.56 $\pm$ 0.01 &   34.89 &  \textbf{37.54} &  2.65 $\pm$ 0.01 \\\midrule
10-shot &  59.67 &  \textbf{61.94} &  2.27 $\pm$ 0.01 &   47.77 &  \textbf{50.81} &  3.04 $\pm$ 0.01 &   41.04 &  \textbf{44.28} &  3.25 $\pm$ 0.01 \\\midrule
\bottomrule
\end{tabular}


==> paper_tables/main/s2m2rf/tritbl_tieredImagenet_val2test_ci.tex <==
% \begin{table}[h]
%   \centering
  
%     \begin{tabular}{ccccccc}
%     \toprule
%             & \multicolumn{3}{c}{5-way} & \multicolumn{3}{c}{10-way} \\\midrule
%             & Before &        After &   Improvement & Before &        After &   Improvement \\\midrule
%     1-shot &  73.50 &  {73.64} $\pm$ 0.25 &  0.14 $\pm$ 0.03 &  61.20 &  {61.44} $\pm$ 0.16 &  0.24 $\pm$ 0.01 \\\midrule
%     5-shot &  88.00 &  {88.31} $\pm$ 0.12 &  0.30 $\pm$ 0.01 &  79.41 &  {80.01} $\pm$ 0.11 &  0.60 $\pm$ 0.01 \\\midrule
%     10-shot &  90.94 &  {91.14} $\pm$ 0.10 &  0.21 $\pm$ 0.01 &  83.88 &  {84.47} $\pm$ 0.09 &  0.58 $\pm$ 0.01 \\
%     \bottomrule
%     \end{tabular}\\ \vspace{0.45em}
    
    
%     \begin{tabular}{ccccccc}
%     \toprule
%             & \multicolumn{3}{c}{15-way} & \multicolumn{3}{c}{20-way} \\\midrule
%             &  Before &        After &   Improvement & Before &        After &   Improvement \\\midrule
%     1-shot & 53.90 &  {53.97} $\pm$ 0.15 &  0.07 $\pm$ 0.01 &  48.81 &  {48.96} $\pm$ 0.11 &  0.15 $\pm$ 0.01 \\\midrule
%     5-shot & 73.33 &  {74.21} $\pm$ 0.09 &  0.88 $\pm$ 0.01 &  68.58 &  {69.71} $\pm$ 0.08 &  1.13 $\pm$ 0.01 \\\midrule
%     10-shot & 78.70 &  {79.57} $\pm$ 0.08 &  0.86 $\pm$ 0.01 &  74.58 &  {75.74} $\pm$ 0.07 &  1.16 $\pm$ 0.01 \\
%     \bottomrule
%     \end{tabular}\\ \vspace{0.45em}
    
%     \begin{tabular}{ccccccc}
%     \toprule
%             & \multicolumn{3}{c}{50-way} & \multicolumn{3}{c}{100-way} \\\midrule
%             & Before &        After &   Improvement &  Before &        After &   Improvement \\\midrule
%     1-shot &  33.91 &  {34.13} $\pm$ 0.06 &  0.22 $\pm$ 0.01 &   24.80 &  {25.00} $\pm$ 0.03 &  0.20 $\pm$ 0.00 \\\midrule
%     5-shot &  52.60 &  {54.71} $\pm$ 0.05 &  2.10 $\pm$ 0.01 &   41.03 &  {43.59} $\pm$ 0.03 &  2.56 $\pm$ 0.01  \\\midrule
%     10-shot &  59.67 &  {61.94} $\pm$ 0.04 &  2.27 $\pm$ 0.01 &   47.77 &  {50.81} $\pm$ 0.02 &  3.04 $\pm$ 0.01 \\
%     \bottomrule
%     \end{tabular}\\ \vspace{0.45em}
    
%     \begin{tabular}{cccc}
%     \toprule
%             & \multicolumn{3}{c}{150-way} \\\midrule
%             & Before &        After &   Improvement \\\midrule
%     1-shot & 20.37 &  {20.56} $\pm$ 0.02 &  0.19 $\pm$ 0.00 \\\midrule
%     5-shot & 34.89 &  {37.54} $\pm$ 0.01 &  2.65 $\pm$ 0.01 \\\midrule
%     10-shot &  41.04 &  {44.28} $\pm$ 0.01 &  3.25 $\pm$ 0.01 \\
%     \bottomrule
%     \end{tabular}\phantom{blahblahblahblahblahblahblahblahblahblah}

    
%   \caption{\textbf{The Firth bias reduction improvements on the tiered-ImageNet dataset shown in Figure~\ref{fig:s2m2rf} of the main paper.} ``Before'' stands for the novel set accuracy without having any Firth bias reduction, and ``After'' stands for the novel set accuracy after applying Firth bias reduction. Note that the confidence intervals are much smaller for the improvement column thanks to the random-effect matching procedure we used in this study. The ``Before'' confidence intervals were similar to the ``After'' confidence intervals, and thus not repeated due to space constraints.}
%   \label{tab:s2m2tieredpart1}%
% \end{table}%

\begin{table}[h]
  \centering
    \begin{tabular}{ccccccc}
    \toprule
    & Before &        After &   Improvement & Before &        After &   Improvement \\\midrule
    & \multicolumn{3}{c}{5-way} & \multicolumn{3}{c}{10-way} \\\midrule
    1-shot &  73.50 &  {73.64} $\pm$ 0.25 &  0.14 $\pm$ 0.03 &  61.20 &  {61.44} $\pm$ 0.16 &  0.24 $\pm$ 0.01 \\\midrule
    5-shot &  88.00 &  {88.31} $\pm$ 0.12 &  0.30 $\pm$ 0.01 &  79.41 &  {80.01} $\pm$ 0.11 &  0.60 $\pm$ 0.01 \\\midrule
    10-shot &  90.94 &  {91.14} $\pm$ 0.10 &  0.21 $\pm$ 0.01 &  83.88 &  {84.47} $\pm$ 0.09 &  0.58 $\pm$ 0.01 \\\midrule
    & \multicolumn{3}{c}{15-way} & \multicolumn{3}{c}{20-way} \\\midrule
    1-shot & 53.90 &  {53.97} $\pm$ 0.15 &  0.07 $\pm$ 0.01 &  48.81 &  {48.96} $\pm$ 0.11 &  0.15 $\pm$ 0.01 \\\midrule
    5-shot & 73.33 &  {74.21} $\pm$ 0.09 &  0.88 $\pm$ 0.01 &  68.58 &  {69.71} $\pm$ 0.08 &  1.13 $\pm$ 0.01 \\\midrule
    10-shot & 78.70 &  {79.57} $\pm$ 0.08 &  0.86 $\pm$ 0.01 &  74.58 &  {75.74} $\pm$ 0.07 &  1.16 $\pm$ 0.01 \\\midrule
    & \multicolumn{3}{c}{50-way} & \multicolumn{3}{c}{100-way} \\\midrule
    1-shot &  33.91 &  {34.13} $\pm$ 0.06 &  0.22 $\pm$ 0.01 &   24.80 &  {25.00} $\pm$ 0.03 &  0.20 $\pm$ 0.00 \\\midrule
    5-shot &  52.60 &  {54.71} $\pm$ 0.05 &  2.10 $\pm$ 0.01 &   41.03 &  {43.59} $\pm$ 0.03 &  2.56 $\pm$ 0.01  \\\midrule
    10-shot &  59.67 &  {61.94} $\pm$ 0.04 &  2.27 $\pm$ 0.01 &   47.77 &  {50.81} $\pm$ 0.02 &  3.04 $\pm$ 0.01 \\\midrule
    & \multicolumn{3}{c}{150-way} \\\midrule
    1-shot & 20.37 &  {20.56} $\pm$ 0.02 &  0.19 $\pm$ 0.00 \\\midrule
    5-shot & 34.89 &  {37.54} $\pm$ 0.01 &  2.65 $\pm$ 0.01 \\\midrule
    10-shot &  41.04 &  {44.28} $\pm$ 0.01 &  3.25 $\pm$ 0.01 \\
    \bottomrule
    \end{tabular}\\ \vspace{0.45em}
  \caption{\textbf{The Firth bias reduction improvements on the tiered-ImageNet dataset shown in Figure~\ref{fig:s2m2rf} in the main paper.} ``Before'' stands for the novel set accuracy without having any Firth bias reduction, and ``After'' stands for the novel set accuracy after applying Firth bias reduction. Note that the confidence intervals are much smaller for the improvement column, thanks to the random-effect matching procedure we used in this study. The ``Before'' confidence intervals were similar to the ``After'' confidence intervals, and thus not repeated due to space constraints.}
  \label{tab:s2m2tieredpart1}%
\end{table}%




==> paper_tables/main/vbb/tritbl_mini_val2test.tex <==
% % Table generated by Excel2LaTeX from sheet 'Sheet2'
% \begin{table}[h]
%   \centering
%     \begin{tabular}{ccccccc}
%     \toprule
%     \multirow{2}[4]{*}{} & \multicolumn{3}{c}{ResNet10} & \multicolumn{3}{c}{ResNet18} \\
% \cmidrule{1-7}          & Before & After & Improvement & Before & After & Improvement \\
%     \midrule
%     1-shot & 7.96 & {7.97}  $\pm$ 0.06 & 0.01  $\pm$ 0.01 & 7.57 & {7.58}  $\pm$ 0.05 & 0.01  $\pm$ 0.01 \\
%     \midrule
%     5-shot & 8.22 & {8.23}  $\pm$ 0.06 & 0.01  $\pm$ 0.01 & 7.94 & {7.95}  $\pm$ 0.06 & 0.01  $\pm$ 0.01 \\
%     \midrule
%     10-shot & 8.19 & {8.24}  $\pm$ 0.05 & 0.06  $\pm$ 0.05 & 8.01 & {8.15}  $\pm$ 0.05 & 0.14  $\pm$ 0.06 \\
%     \midrule
%     15-shot & 8.21 & {8.36}  $\pm$ 0.05 & 0.15  $\pm$ 0.06 & 8.09 & {8.47}  $\pm$ 0.05 & 0.38  $\pm$ 0.06 \\
%     \midrule
%     20-shot & 8.22 & {8.51}  $\pm$ 0.05 & 0.28  $\pm$ 0.06 & 8.15 & {8.75}  $\pm$ 0.06 & 0.60  $\pm$ 0.06 \\
%     \midrule
%     25-shot & 8.25 & {8.51}  $\pm$ 0.05 & 0.25  $\pm$ 0.06 & 8.27 & {8.92}  $\pm$ 0.05 & 0.65  $\pm$ 0.06 \\
%     \bottomrule
%     \end{tabular}\\ \vspace{0.45em}
%     \begin{tabular}{ccccccc}
%     \toprule
%     \multirow{2}[4]{*}{} & \multicolumn{3}{c}{ResNet34} & \multicolumn{3}{c}{ResNet50} \\
% \cmidrule{1-7}          & Before & After & Improvement & Before & After & Improvement \\
%     \midrule
%     1-shot & 7.47 & {7.48}  $\pm$ 0.05 & 0.01  $\pm$ 0.01 & 7.51 & {7.52}  $\pm$ 0.05 & 0.01  $\pm$ 0.01 \\
%     \midrule
%     5-shot & 7.69 & {7.70}  $\pm$ 0.05 & 0.01  $\pm$ 0.01 & 7.73 & {7.78}  $\pm$ 0.05 & 0.05  $\pm$ 0.05 \\
%     \midrule
%     10-shot & 7.73 & {7.96}  $\pm$ 0.05 & 0.23  $\pm$ 0.05 & 7.83 & {8.59}  $\pm$ 0.05 & 0.76  $\pm$ 0.06 \\
%     \midrule
%     15-shot & 7.79 & {8.22}  $\pm$ 0.05 & 0.43  $\pm$ 0.06 & 7.89 & {9.02}  $\pm$ 0.05 & 1.13  $\pm$ 0.06 \\
%     \midrule
%     20-shot & 7.87 & {8.41}  $\pm$ 0.05 & 0.55  $\pm$ 0.06 & 8.15 & {9.67}  $\pm$ 0.06 & 1.52  $\pm$ 0.06 \\
%     \midrule
%     25-shot & 7.97 & {8.54}  $\pm$ 0.05 & 0.57  $\pm$ 0.06 & 8.44 & {10.71}  $\pm$ 0.06 & 2.27  $\pm$ 0.06 \\
%     \bottomrule
%     \end{tabular}\\ \vspace{0.45em}
%     \begin{tabular}{cccc}
%     \toprule
%     \multirow{2}[4]{*}{} & \multicolumn{3}{c}{ResNet101} \\
% \cmidrule{1-4}          & Before & After & Improvement \\
%     \midrule
%     1-shot & 7.63 & {7.65}  $\pm$ 0.05 & 0.02  $\pm$ 0.02 \\
%     \midrule
%     5-shot & 7.81 & {7.88}  $\pm$ 0.05 & 0.07  $\pm$ 0.05 \\
%     \midrule
%     10-shot & 7.96 & {8.81}  $\pm$ 0.05 & 0.86  $\pm$ 0.06 \\
%     \midrule
%     15-shot & 8.10 & {9.50}  $\pm$ 0.05 & 1.40  $\pm$ 0.06 \\
%     \midrule
%     20-shot & 8.37 & {10.29}  $\pm$ 0.06 & 1.91  $\pm$ 0.06 \\
%     \midrule
%     25-shot & 8.74 & {10.62}  $\pm$ 0.06 & 1.88  $\pm$ 0.06 \\
%     \bottomrule
%     \end{tabular}\phantom{blahblahblahblahblahblahblahblahblahbl}%
%   \label{tab:addlabel}%
%   \caption{\textbf{The Firth bias reduction improvements on the mini-ImageNet dataset shown in Figure~\ref{fig:firthvsl2lin} of the main paper.} ``Before'' stands for the novel set accuracy without having any Firth bias reduction, and ``After'' stands for the novel set accuracy after applying Firth bias reduction. Note that the confidence intervals are much smaller for the improvement column thanks to the random-effect matching procedure we used in this study. The ``Before'' confidence intervals were similar to the ``After'' confidence intervals, and thus not repeated due to space constraints.}\label{tab:resnet-mini-absacc}
% \end{table}%

% Table generated by Excel2LaTeX from sheet 'Sheet2'
\begin{table}[h]
  \centering
    \begin{tabular}{ccccccc}
    \toprule
    \cmidrule{1-7}          & Before & After & Improvement & Before & After & Improvement \\\midrule
    \multirow{2}[4]{*}{} & \multicolumn{3}{c}{ResNet10} & \multicolumn{3}{c}{ResNet18} \\
    \midrule
    1-shot & 7.96 & {7.97}  $\pm$ 0.06 & 0.01  $\pm$ 0.01 & 7.57 & {7.58}  $\pm$ 0.05 & 0.01  $\pm$ 0.01 \\
    \midrule
    5-shot & 8.22 & {8.23}  $\pm$ 0.06 & 0.01  $\pm$ 0.01 & 7.94 & {7.95}  $\pm$ 0.06 & 0.01  $\pm$ 0.01 \\
    \midrule
    10-shot & 8.19 & {8.24}  $\pm$ 0.05 & 0.06  $\pm$ 0.05 & 8.01 & {8.15}  $\pm$ 0.05 & 0.14  $\pm$ 0.06 \\
    \midrule
    15-shot & 8.21 & {8.36}  $\pm$ 0.05 & 0.15  $\pm$ 0.06 & 8.09 & {8.47}  $\pm$ 0.05 & 0.38  $\pm$ 0.06 \\
    \midrule
    20-shot & 8.22 & {8.51}  $\pm$ 0.05 & 0.28  $\pm$ 0.06 & 8.15 & {8.75}  $\pm$ 0.06 & 0.60  $\pm$ 0.06 \\
    \midrule
    25-shot & 8.25 & {8.51}  $\pm$ 0.05 & 0.25  $\pm$ 0.06 & 8.27 & {8.92}  $\pm$ 0.05 & 0.65  $\pm$ 0.06 \\\midrule
    \multirow{2}[4]{*}{} & \multicolumn{3}{c}{ResNet34} & \multicolumn{3}{c}{ResNet50} \\
    \midrule
    1-shot & 7.47 & {7.48}  $\pm$ 0.05 & 0.01  $\pm$ 0.01 & 7.51 & {7.52}  $\pm$ 0.05 & 0.01  $\pm$ 0.01 \\
    \midrule
    5-shot & 7.69 & {7.70}  $\pm$ 0.05 & 0.01  $\pm$ 0.01 & 7.73 & {7.78}  $\pm$ 0.05 & 0.05  $\pm$ 0.05 \\
    \midrule
    10-shot & 7.73 & {7.96}  $\pm$ 0.05 & 0.23  $\pm$ 0.05 & 7.83 & {8.59}  $\pm$ 0.05 & 0.76  $\pm$ 0.06 \\
    \midrule
    15-shot & 7.79 & {8.22}  $\pm$ 0.05 & 0.43  $\pm$ 0.06 & 7.89 & {9.02}  $\pm$ 0.05 & 1.13  $\pm$ 0.06 \\
    \midrule
    20-shot & 7.87 & {8.41}  $\pm$ 0.05 & 0.55  $\pm$ 0.06 & 8.15 & {9.67}  $\pm$ 0.06 & 1.52  $\pm$ 0.06 \\
    \midrule
    25-shot & 7.97 & {8.54}  $\pm$ 0.05 & 0.57  $\pm$ 0.06 & 8.44 & {10.71}  $\pm$ 0.06 & 2.27  $\pm$ 0.06 \\\midrule
    \multirow{2}[4]{*}{} & \multicolumn{3}{c}{ResNet101} \\\midrule
    1-shot & 7.63 & {7.65}  $\pm$ 0.05 & 0.02  $\pm$ 0.02 \\
    \midrule
    5-shot & 7.81 & {7.88}  $\pm$ 0.05 & 0.07  $\pm$ 0.05 \\
    \midrule
    10-shot & 7.96 & {8.81}  $\pm$ 0.05 & 0.86  $\pm$ 0.06 \\
    \midrule
    15-shot & 8.10 & {9.50}  $\pm$ 0.05 & 1.40  $\pm$ 0.06 \\
    \midrule
    20-shot & 8.37 & {10.29}  $\pm$ 0.06 & 1.91  $\pm$ 0.06 \\
    \midrule
    25-shot & 8.74 & {10.62}  $\pm$ 0.06 & 1.88  $\pm$ 0.06 \\
    \bottomrule
    \end{tabular}\\ \vspace{0.45em}
  \label{tab:addlabel}%
  \caption{\textbf{The Firth bias reduction improvements on the mini-ImageNet dataset shown in Figure~\ref{fig:firthvsl2lin} in the main paper.} ``Before'' stands for the novel set accuracy without having any Firth bias reduction, and ``After'' stands for the novel set accuracy after applying Firth bias reduction. Note that the confidence intervals are much smaller for the improvement column, thanks to the random-effect matching procedure we used in this study. The ``Before'' confidence intervals were similar to the ``After'' confidence intervals, and thus not repeated due to space constraints.}\label{tab:resnet-mini-absacc}
\end{table}%
